Learning Scalable and Precise Representation of Program Semantics

Neural program embedding has shown potential in aiding the analysis of large-scale, complicated software. Newly proposed deep neural architectures pride themselves on learning program semantics rather than superficial syntactic features. However, by considering the source code only, the vast majority of neural networks do not capture a deep, precise representation of program semantics. In this paper, we present \dypro, a novel deep neural network that learns from program execution traces. Compared to the prior dynamic models, not only is \dypro capable of generalizing across multiple executions for learning a program's dynamic semantics in its entirety, but \dypro is also more efficient when dealing with programs yielding long execution traces. For evaluation, we task \dypro with semantic classification (i.e. categorizing programs based on their semantics) and compared it against two prominent static models: Gated Graph Neural Network and TreeLSTM. We find that \dypro achieves the highest prediction accuracy among all models. To further reveal the capacity of all aforementioned deep neural architectures, we examine if the models can learn to detect deeper semantic properties of a program. In particular given a task of recognizing loop invariants, we show \dypro beats all static models by a wide margin.

==> discuss.tex <==
\section{Results and Discussion}
\label{sec:res}
In this section, we present our evaluation results 
together with a in-depth discussion.

\subsection{Accuracy}
Figure~\ref{fig:accu} shows the prediction accuracy of 
the four models. As depicted, all models are very accurate 
in classifying the functionality confirming the hypothesis 
the three deep neural networks match the baseline model 
TreeLSTM. However, regarding semantic classifications all models except 
\dypro suffer notable drops. TreeLSTM hardly manages 50\% while 
the other two are under 70\%. In terms of the precision, recall 
and F1 scores, \dypro also achieves significantly better 
results than all others (Table~\ref{table:pr}). To understand 
the cause of lower accuracy in static models, 
we conduct a comprehensive inspection on their performance 
\wrt hand-picked test data and summarize our 
findings below.

\begin{figure}[ht!]
	\vskip 0.1in
	\begin{center}
		\centerline{\includegraphics[width=\columnwidth]{figures/accuracy}}
		\caption{Model Accuracy.}
		\label{fig:accu}
	\end{center}
	\vskip -0.3in
\end{figure}

\begin{table}[ht!]
		\vskip 0.07in
		\begin{center}
		\begin{adjustbox}{max width=\columnwidth}
		\begin{tabular}{c  c  c  c }
			\hline
%			\multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c|}{\textit{Micro Averaged}} & \multicolumn{3}{c}{\textit{Macro Averaged}}  \\\cline{2-7}
%			& Precision & Recall & F1 Score & Precision & Recall & F1 Score \\
			\textbf{Models} &\textbf{Precision} &\textbf{Recall} &\textbf{F1 Score} \\
			\hline
			TreeLSTM &0.57 &0.53 &0.54 \\
			\hline
			\begin{tabular}{@{}c@{}} Gated Graph \\ Neural Network \end{tabular} &0.69 &0.66 &0.67 \\
			\hline
			\begin{tabular}{@{}c@{}} AST Path \\ Neural Network \end{tabular} &0.64 &0.58 &0.6\\
			\hline
			\hline
			\textbf{\dypro}  &\textbf{0.86} &\textbf{0.81} &\textbf{0.83} \\
			\hline	
		\end{tabular}
		\end{adjustbox}
	\end{center}
	\caption{Precision, recall and F1 score of all models. All scores are macro averaged. Micro average gives very similar results which we ignore for brevity.  }
	\label{table:pr}
%		\vskip -0.3in
\end{table}
%\vspace*{.4cm}

\begin{figure*}[ht!]
	\begin{subfigure}[b]{0.32\textwidth}
		\lstset{style=mystyle}
		\lstinputlisting[escapechar=@,basicstyle=\linespread{.90}\fontsize{7}{11.2}\ttfamily]{figures/53.cs}	
		\vspace{-.3cm}	
		\caption{}
		\label{fig:ss1}
	\end{subfigure}
	\; %\quad
	\begin{subfigure}[b]{0.32\textwidth}		
		\lstset{style=mystyle}
		\lstinputlisting[escapechar=@,basicstyle=\linespread{.85}\fontsize{7}{11.2}\ttfamily]{figures/190.cs}	
		\vspace{-.3cm}	
		\caption{}
		\label{fig:ss2}
	\end{subfigure}
	\; %\quad
	\begin{subfigure}[b]{0.32\textwidth}
		\lstset{style=mystyle}
		\lstinputlisting[escapechar=@,basicstyle=\linespread{.85}\fontsize{7}{11.2}\ttfamily]{figures/221.cs}	
		\vspace{-.3cm}	
		\caption{}
		\label{fig:ss3}
	\end{subfigure}
	\begin{subfigure}[b]{0.32\textwidth}
		\lstset{style=mystyle}
		\lstinputlisting[escapechar=@,basicstyle=\linespread{.85}\fontsize{7}{11.2}\ttfamily]{figures/310.cs}		
		\vspace{-.3cm}	
		\caption{}
		\label{fig:ss4}
	\end{subfigure}
	\; %\quad
	\begin{subfigure}[b]{0.32\textwidth}		
		\lstset{style=mystyle}
		\lstinputlisting[escapechar=@,basicstyle=\linespread{1}\fontsize{7}{11.2}\ttfamily]{figures/324.cs}	
		\vspace{-.3cm}	
		\caption{}
		\label{fig:ss5}
	\end{subfigure}
	\; %\quad
	\begin{subfigure}[b]{0.32\textwidth}
		\lstset{style=mystyle}
		\lstinputlisting[escapechar=@,basicstyle=\linespread{1}\fontsize{7}{11.2}\ttfamily]{figures/388.cs}	
		\vspace{-.3cm}	
		\caption{}
		\label{fig:ss6}
	\end{subfigure}
	\caption{Syntactically different but semantically equivalent programs.}
	\label{fig:ss}
	\vskip -0.1in
\end{figure*}

\paragraph{\textbf{Different Syntax, Same Semantics}} 
Static models have performed poorly against programs 
that are syntactically different but semantically 
equivalent. Given the six programs shown in Figure~\ref{fig:ss}, 
gated graph neural network predicted two correctly (Figure~\ref{fig:ss1} 
and~\ref{fig:ss3}), and three different 
labels in total. Similarly, 
AST path neural network predicted three programs correctly 
(Figure~\ref{fig:ss1}, Figure~\ref{fig:ss2} and~\ref{fig:ss3}) 
and four different labels in total. However, they both 
performed better than TreeLSTM which produced only one 
correct prediction (Figure~\ref{fig:ss5}) and three labels 
in total. This phenomenon is a clear indication the 
static models do not capture a precise representation of 
program semantics in their embeddings (\ie they do not learn to 
interpret the computation in the numerical space), instead they 
still focus on mining the syntactic patterns. Due to their superior 
expressiveness with the extra feature dimensions, they 
outperform a model that learns from program syntax only such 
as TreeLSTM. On the contrary, \dypro correctly predicted all six 
programs with a single label. The reason being \dypro learns from program 
executions, in other words, \dypro discovers the semantic patterns 
from the runtime information which apparently canonicalize the 
syntactic variations. 

\paragraph{\textbf{Similar Syntax, Different Semantics}} 
Static models also struggled to differentiate different 
semantics for programs of similar syntax, especially 
when source code differ in only several tokens such as those depicted in 
Figure~\ref{fig:ds1} and~\ref{fig:ds2}. All three models 
considered the two programs semantically equivalent 
even though program in Figure~\ref{fig:ds1} adopts bubble sort while 
Figure~\ref{fig:ds2} adopts insertion sort. A further 
evidence to show the embeddings they learn do not capture a 
precise representation of program semantics. 


\begin{figure}[ht!]
	\begin{subfigure}[b]{0.23\textwidth}
		\lstset{style=mystyle}
		\lstinputlisting[basicstyle=\linespread{.80}\fontsize{6}{8.8}\ttfamily]{figures/diff1.cs}		
		\vspace{-.3cm}	
		\caption{}
		\label{fig:ds1}
	\end{subfigure}
	\;
	\begin{subfigure}[b]{0.23\textwidth}		
		\lstset{style=mystyle}
		\lstinputlisting[basicstyle=\linespread{.80}\fontsize{6}{8.8}\ttfamily]{figures/diff2.cs}	
		\vspace{-.3cm}	
		\caption{}
		\label{fig:ds2}
	\end{subfigure}
	\caption{Syntactically similar but semantically different programs. Textual differences are highlighted in red box.}
	\label{fig:ds}
\end{figure}


\paragraph{\textbf{Performance Profiling for \dypro}} 
Apparently, \dypro won't be trapped by the aforementioned 
situations. Instead, \dypro's inaccuracies mainly stems 
from the reduction of program states. At one extreme, if 
\dypro keeps all the program states, its accuracy would 
exceed 95\%. As more states being reduced, misclassifications 
increases when reaching the other extreme at which the states 
become too few for \dypro to learn anything meaningful.
%However, due to its conflicting objective functions 
%in the training phase, \dypro needs to strike a balance 
%between prediction accuracy and reduction effectiveness. 
%Hence, it can be inaccurate when it over-reduces the program 
%states to the degree it's unable to learn the semantic property 
%of an execution. 
We capture a number of training epochs 
to demonstrate how \dypro's accuracy/F1 score changes 
with a increasing reduction rate of program states (Figure~\ref{fig:reacc}/Figure~\ref{fig:ref1}). 
We also conduct a separate experiment to compare the 
generalization procedure among all models. Our intuition is 
a large number of surface-level syntactic discrepancies 
will be automatically unified into the same execution. 
As a result, it decreases the amount of training data 
\dypro needs compared to the static models. Figure~\ref{fig:retrac} 
and~\ref{fig:retrf1} show the results, as we randomly reduce the training data, 
up to 66\%/69\% of the original set, \dypro still performed slightly better 
than all the static models \wrt accuracy/F1 score. 


\begin{figure}[ht!]
	\nocaption
	\begin{subfigure}[b]{0.23\textwidth}
		\centerline{\includegraphics[width=\columnwidth]{figures/reacc}}
		\caption{How prediction accuracy vary with the reduction rate.}
		\label{fig:reacc}
	\end{subfigure}
	\;
	\begin{subfigure}[b]{0.23\textwidth}		
		\centerline{\includegraphics[width=\columnwidth]{figures/ref1}}
		\caption{How F1 score vary with the reduction rate.}
		\label{fig:ref1}
	\end{subfigure}
%	\caption{}
%	\label{}
\end{figure}


\begin{figure}[ht!]
	\nocaption
	\begin{subfigure}[b]{0.23\textwidth}
		\centerline{\includegraphics[width=\columnwidth]{figures/retrac}}
		\caption{Accuracy trend as training data decreases.}
		\label{fig:retrac}
	\end{subfigure}
	\;
	\begin{subfigure}[b]{0.23\textwidth}		
		\centerline{\includegraphics[width=\columnwidth]{figures/retrf1}}
		\caption{F1 score trend as training data decreases.}
		\label{fig:retrf1}
	\end{subfigure}
	%	\caption{}
	%	\label{}
\end{figure}


\subsection{Robustness}
We propose the robustness metric to measure how stable the 
models are with their prediction results. As mentioned in 
Section~\ref{subsec:coset}, we apply semantically preserving 
transformations to programs in the testing set that are 
correctly predicted before, and then examine 
if static models would predict differently against 
the new test set. As for \dypro we randomly inject new variables 
and statements into the test programs and investigate if such 
changes will have any influence on the model prediction.  

In general, the code transformations hurt the model 
predictions. Figure~\ref{fig:robust} depicts on average how many 
programs that are correctly predicted before being misclassified 
due to the transformations. As the number of transformations 
increases to three and more, the overall accuracy of all static 
models drop to below 50\%. In particular we disclose one transformation 
that contributed the most to the decline of model accuracy. 


\begin{figure}[ht!]
	\begin{center}
		\centerline{\includegraphics[width=\columnwidth]{figures/robust}}
		\caption{Number of misclassifications due to transformations.}
		\label{fig:robust}
	\end{center}
	\vskip -0.2in
\end{figure}

Given a program, we incorporate adversarial statements that are frequently 
appeared in programs of different semantics. However, in 
order to preserve the original semantics of the program, we use 
control statements such as \textit{if} or \textit{for} statements to prevent 
the adversarial statements from being executed. Figure~\ref{fig:roco} shows an 
example. The idea is if a model learns to interpret the program 
semantics, it would have some knowledge on how a control statement 
would govern the program execution \eg execute a branch only if 
the condition is evaluated to be true or repeatedly 
execute the loop body until the condition is no longer met. 
Instead, if a model only learns to capture the syntactic 
patterns, it would likely to be fooled by the adversarial statements 
that are representative features of the other labels. We find 
out all static models have a severe difficulty in dealing with 
the transformation. A large number of programs managed to 
mislead them to the wrong predictions (Figure~\ref{fig:robust2}). 

\begin{figure}[ht!]
	\lstset{style=mystyle}
	\lstinputlisting[basicstyle=\linespread{.80}\fontsize{7}{11.2}\ttfamily,numbers=none]{figures/robust.cs}	
	\vspace{-.3cm}	
	\caption{An example of showing how to preserve the program semantics while adding the adversarial statements. Statements added are highlighted in red.
	}
	\label{fig:roco}
\end{figure}


\begin{figure}[ht!]
	\begin{center}
		\centerline{\includegraphics[width=\columnwidth]{figures/robust2}}
		\caption{Revealing the impact of adversarial statements.}
		\label{fig:robust2}
	\end{center}
%	\vskip -0.4in
\end{figure}


To evaluate the robustness of \dypro, we also mixed statements 
in programs of different semantics. Unlike the previous 
experiments, added statements will be executed leading to the 
change of program semantics, however, those added statements 
are not heavily involved in the computation, ideally, \dypro 
should not change its prediction. To draw a comparison, we test 
all four models\footnote{Static models work with the source code 
while \dypro is tested against the executions of the same programs.} and present the results in Figure~\ref{fig:sc}. 
As states capacity (\ie number of variables in each program 
state times the total number of program states in an execution) 
) increases, \dypro is shown to be stable with its predictions. 
When under 30\% increase, \dypro maintained its prediction for 
the vast majority of the programs that are correctly predicted 
before. Compared to \dypro, static models are much more likely 
to sway their predictions.

\begin{figure}[ht!]
	\begin{center}
		\centerline{\includegraphics[width=\columnwidth]{figures/sc}}
		\caption{Model predictions \wrt the increase of state capacity.}
		\label{fig:sc}
	\end{center}
	\vskip -0.35in
\end{figure}


\subsection{Concluding Remarks}
In this section, we have given a detailed discussion on 
the strength and weakness of each model. To summarize, 
despite the considerable progress, static models 
are shown to be limited in learning the representation of 
program semantics. It is evident their generalization still 
happens at the level of program syntax, manifested in the 
difficulty of unifying program semantics among syntactic 
variations or differentiating program semantics with syntactic 
similarities. However, due to the superior model architecture 
and more informative program representation, they are able 
to learn more complex, fine-grained syntactic features that 
a pure syntactic model can't. On the other hand, \dypro 
learns from program executions, a more direct and concrete 
representation of program semantics. Therefore \dypro is able to 
learn a more precise interpretation of programs by discovering 
the patterns at the semantic level. To cope with the infamous 
scalability issue of any dynamic approach, we incorporate the 
states reduction mechanism to \dypro so it only generalizes from the 
key program states while discarding the peripherals. Also worth 
noting, even if we did not demonstrate the utility of 
\dypro in specific problem settings, given its capability 
of learning precise representations of program semantics, \dypro 
should be readily applicable to many downstream programming 
tasks such as bug localization, repair generation, variable name 
or method name prediction. 





%
%
%
%
%
%
% 
%
%
%
%
%
%
%
%
%
%
%
%
%
%Regarding measurement of model robustness, 
%%we pick the programs that have been predicted correctly by each 
%%model to generate variants. Here we provide the details of this procedure. 
%first, for each correctly predicted program by each model, we randomly apply our local 
%transformation rules\footnote{Readers 
%are encouraged to consult the supplementary material for the 
%details of all transformation rules.} to generate a mutant. Then we collect all mutants 
%to form a new test set for each model to predict respectively. For the 
%mutants that have been predicted incorrectly, we remove them from the 
%new test set and register their scores based on the discrepancies (\ie the 
%number of tokens) between the original program and current version of the 
%mutant. If the mutants are being predicted correctly, we will continue to apply 
%more transformations to test the models. The whole process stops until there 
%is no mutants left in the test set, in which case we average over the 
%scores among all mutants as the robustness score for each model. 
%Figure~\ref{fig:rob} depicted the results.
%
%
%
%
%
%
%
%\begin{figure}[ht]
%\vskip 0.2in
%\begin{center}
%\centerline{\includegraphics[width=\columnwidth]{robustness}}
%\caption{Model Robustness.}
%\label{fig:rob}
%\end{center}
%\vskip -0.2in
%\end{figure}
%
%
%
%
%Scalability is always an important metric to measure the quality of 
%any program analysis technique. Here we disclose how each model 
%fare against the increasing size or execution traces of programs. 
%
%Figure~\ref{fig:sca} and~\ref{fig:scad} shows how the accuracy of each model changes as 
%the program size or execution trace increases.
%
%\begin{figure}[ht]
%\vskip 0.2in
%\begin{center}
%\centerline{\includegraphics[width=\columnwidth]{sca}}
%\caption{Model Scalability.}
%\label{fig:sca}
%\end{center}
%\vskip -0.2in
%\end{figure}
%
%\begin{figure}[ht]
%\vskip 0.2in
%\begin{center}
%\centerline{\includegraphics[width=\columnwidth]{scadypro}}
%\caption{\dypro Scalability.}
%\label{fig:scad}
%\end{center}
%\vskip -0.2in
%\end{figure}
%
%
%%Similarly, Figure~\ref{} and~\ref{} shows the trend of model robustness. 
%
%
%We also conducted another experiment to investigate \dypro's capability of 
%compressing execution traces. As shown in Figure~\ref{fig:com}, \dypro consistently 
%discarded more than 50\% of the program states.
%
%
%\begin{figure}[ht]
%\vskip 0.2in
%\begin{center}
%\centerline{\includegraphics[width=\columnwidth]{compress}}
%\caption{\dypro's compression of execution traces.}
%\label{fig:com}
%\end{center}
%\vskip -0.2in
%\end{figure}


==> related.tex <==
\section{Related Work}
\label{sec:rela}
%In this section, we survey two lines of related work in the literature. 
\paragraph{Learning Program Representations}
\citet{hindle2012naturalness} pioneered the field of 
learning language models from source code. A significant finding 
of theirs is programs, similar to natural language, are highly 
repetitive and predictable. With the rapid development of deep learning techniques and the increasing 
accessibility of large scale open source code repository, many works begin 
to apply deep neural networks to learn syntactic program representations
~\cite{gupta2017deepfix,pu2016sk_p,maddison2014structured,bielik2016phog,mou2016convolutional}. 
More recently, a new line of research emerges aiming to tackle the problem of 
learning semantic representation~\cite{wang2017dynamic,henkel2018code,allamanis2017learning,DeFreez,alon2018code2vec}. 
In this paper we present \dypro, a novel dynamic model that learns program 
semantics from execution traces. Our evaluation shows \dypro is more accurate in understanding 
and analyzing program semantics than several prominent static models.

\paragraph{Learning from Execution Traces}
Learning from execution traces also shows promise in the 
domain of program synthesis. Neural program interpreter (NPI)~\cite{reed2015neural}
is the first to learn to execute programs given their execution traces.~\citet{cai2017making} 
further improves NPI's generalization capability via 
recursion. Shin~\etal propose a new deep neural architecture to learn 
to synthesis programs~\cite{shin2018improving}. 
%Their models work in two steps. First 
%given the input-output examples, it infers the execution trace. 
%Then it uses execution trace to infer the program. 
A fundamental 
difference between \dypro and those attempts is \dypro learns 
from the sequence of program states created by the execution whereas
they use execution trace in pure syntax.  

